Unearthing Large Scale Domain-Specific Knowledge from Public Corpora

Large language models (LLMs) have demonstrated remarkable potential in various tasks, however, there remains a significant lack of open-source models and data for specific domains. Previous work has primarily focused on manually specifying resources and collecting high-quality data for specific domains, which is extremely time-consuming and labor-intensive. To address this limitation, we introduce large models into the data collection pipeline to guide the generation of domain-specific information and retrieve relevant data from Common Crawl (CC), a large public corpus. We refer to this approach as Retrieve-from-CC. It not only collects data related to domain-specific knowledge but also mines the data containing potential reasoning procedures from the public corpus. By applying this method, we have collected a knowledge domain-related dataset named Retrieve-Pile, which covers four main domains, including the sciences, humanities, and other categories. Through the analysis of , Retrieve-from-CC can effectively retrieve relevant data from the covered knowledge domains and significantly improve the performance in tests of mathematical and knowledge-related reasoning abilities. We have released Retrieve-Pile at https://huggingface.co/datasets/Query-of-CC/Retrieve-Pile.

==> latex/bak.tex <==
% \section{More detailed results}

% \subsection{Math}

% \begin{table*}[!tbp]
%   \centering
%   \resizebox{\textwidth}{!}{
%     \begin{tabular}{cp{1.44em}cccccccc}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{m{5em}}{\textbf{Number Theory}} & \multicolumn{1}{m{6.625em}}{\textbf{Counting\& Probability}} & \multicolumn{1}{m{6.065em}}{\textbf{Intermediate Algebra}} & \textbf{Algebra} & \textbf{Geometry} & \textbf{Prealgebra} & \textbf{Precalculus} & \textbf{Average} \\
%     \midrule
%     Llama2 & 7B    & 2.78  & 2.74  & 1.77  & 3.88  & 2.92  & 6.08  & 1.83  & 3.14  \\
%     Llama2-QoC & 7B    & 4.07\tiny{(+46.67\%)} & 4.01\tiny{(+46.15\%)} & 2.88\tiny{(+62.50\%)} & 8.85\tiny{(+128.26\%)} & 4.59\tiny{(+57.14\%)} & 11.25\tiny{(+84.91\%)} & 3.3\tiny{(+80.00\%)} & 5.56\tiny{(+76.98\%)} \\
%     \midrule
%     Mistral  & 7B    & 7.22  & 6.54  & 5.32  & 18.20  & 7.72  & 19.75  & 4.03  & 9.83  \\
%     Mistral-QoC & 7B    & 11.3\tiny{(+56.41\%)} & 11.39\tiny{(+74.19\%)} & 7.53\tiny{(+41.67\%)} & 28.05\tiny{(+54.17\%)} & 13.15\tiny{(+70.27\%)} & 29.85\tiny{(+51.16\%)} & 6.41\tiny{(+59.09\%)} & 15.38\tiny{(+56.58\%)} \\
%     \bottomrule
%     \end{tabular}%
%   }
%   \caption{Add caption}\label{tab:addlabel}%
% \end{table*}%


% \subsection{MMLU}

% \begin{table*}[!tbp]
%   \centering
%   \resizebox{\textwidth}{!}{
%     \begin{tabular}{lccccccc}
%     \toprule
%           & Llama 2 & CodeLlama & Llemma & Qwen 2 & Mistral & Llama2-QoC & Mistral-QoC \\
%           & 7B    & 7B    & 7B    & 7B    & 7B    & 7B    & 7B \\
%     \midrule
%     abstract algebra & 29.00  & 22.00  & 20.00  & 33.00  & 29.00  & 24.00  & \textbf{35.00 } \\
%     anatomy & 47.41  & 32.59  & 40.00  & 49.63  & \textbf{62.96 } & 51.85  & 60.74  \\
%     astronomy & 40.79  & 32.24  & 59.21  & 64.47  & 65.79  & 56.58  & \textbf{73.03 } \\
%     business ethics & 53.00  & 44.00  & 50.00  & 69.00  & 57.00  & 57.00  & \textbf{70.00 } \\
%     clinical knowledge & 46.04  & 40.00  & 49.81  & 62.26  & 69.43  & 59.25  & \textbf{70.57 } \\
%     college biology & 46.53  & 34.72  & 48.61  & 67.36  & 72.92  & 63.89  & \textbf{77.08 } \\
%     college chemistry & 34.00  & 29.00  & 44.00  & 47.00  & \textbf{50.00 } & 43.00  & 48.00  \\
%     college computer science & 33.00  & 42.00  & 45.00  & \textbf{53.00 } & 52.00  & 46.00  & 51.00  \\
%     college mathematics & 35.00  & 28.00  & 36.00  & 28.00  & 40.00  & 37.00  & \textbf{43.00 } \\
%     college medicine & 42.20  & 35.26  & 47.40  & 58.96  & 65.32  & 58.38  & \textbf{67.63 } \\
%     college physics & 22.55  & 17.65  & 34.31  & 40.20  & 38.24  & 37.25  & \textbf{42.16 } \\
%     computer security & 60.00  & 55.00  & 65.00  & 73.00  & \textbf{77.00 } & 69.00  & \textbf{77.00 } \\
%     conceptual physics & 42.55  & 34.04  & 46.81  & 52.77  & 57.02  & 50.64  & \textbf{63.83 } \\
%     econometrics & 28.95  & 30.70  & 35.96  & 32.46  & \textbf{50.00 } & 42.11  & 45.61  \\
%     electrical engineering & 48.28  & 46.21  & 56.55  & 57.24  & 57.93  & 55.86  & \textbf{70.34 } \\
%     elementary mathematics & 27.25  & 30.16  & 44.18  & 43.65  & 37.83  & 32.28  & \textbf{48.68 } \\
%     formal logic & 27.78  & 29.37  & 39.68  & 44.44  & 41.27  & 33.33  & \textbf{50.79 } \\
%     global facts & 32.00  & 30.00  & 24.00  & 37.00  & 36.00  & 38.00  & \textbf{39.00 } \\
%     high school biology & 50.97  & 40.00  & 50.97  & 71.94  & 76.77  & 66.77  & \textbf{79.68 } \\
%     high school chemistry & 36.95  & 31.03  & 47.29  & 51.23  & \textbf{53.20 } & 41.87  & \textbf{53.20 } \\
%     high school computer science & 40.00  & 49.00  & 59.00  & 68.00  & 68.00  & 55.00  & \textbf{71.00 } \\
%     high school european history & 60.61  & 46.67  & 50.91  & 67.27  & \textbf{78.79 } & 69.70  & 73.94  \\
%     high school geography & 48.99  & 45.96  & 55.05  & 75.76  & 76.77  & 72.73  & \textbf{81.82 } \\
%     high school government and politics & 67.36  & 49.22  & 53.37  & 83.94  & 86.53  & 78.24  & \textbf{91.71 } \\
%     high school macroeconomics & 45.90  & 36.15  & 47.69  & 60.00  & \textbf{66.15 } & 56.41  & 65.90  \\
%     high school mathematics & 29.63  & 24.07  & 33.33  & 30.00  & 33.70  & 28.52  & \textbf{34.44 } \\
%     high school microeconomics & 44.54  & 36.97  & 50.42  & 59.24  & 66.39  & 55.88  & \textbf{73.53 } \\
%     high school physics & 31.79  & 37.75  & 38.41  & 37.75  & 32.45  & 35.76  & \textbf{40.40 } \\
%     high school psychology & 62.57  & 47.34  & 62.57  & 79.27  & 82.39  & 78.72  & \textbf{84.59 } \\
%     high school statistics & 27.31  & 42.13  & 43.98  & 44.44  & \textbf{57.41 } & 45.37  & 52.31  \\
%     high school us history & 60.29  & 48.04  & 49.51  & 75.98  & \textbf{78.92 } & 72.55  & 75.98  \\
%     high school world history & 62.87  & 53.59  & 57.81  & 75.95  & \textbf{77.22 } & 74.26  & \textbf{77.22 } \\
%     human aging & 56.05  & 37.67  & 40.81  & 63.23  & 69.96  & 61.88  & \textbf{72.65 } \\
%     human sexuality & 54.96  & 44.27  & 49.62  & 69.47  & \textbf{78.63 } & 70.23  & 77.86  \\
%     international law & 65.29  & 49.59  & 61.16  & 76.86  & 77.69  & 74.38  & \textbf{83.47 } \\
%     jurisprudence & 53.70  & 44.44  & 52.78  & 73.15  & 77.78  & 64.81  & \textbf{81.48 } \\
%     logical fallacies & 50.92  & 35.58  & 53.99  & 66.26  & 79.14  & 69.33  & \textbf{79.75 } \\
%     machine learning & 38.39  & 36.61  & 33.93  & 37.50  & 49.11  & 43.75  & \textbf{54.46 } \\
%     management & 54.37  & 52.43  & 61.17  & 77.67  & \textbf{82.52 } & 71.84  & 79.61  \\
%     marketing & 68.38  & 63.68  & 68.38  & 83.76  & 87.61  & 82.91  & \textbf{91.03 } \\
%     medical genetics & 55.00  & 41.00  & 54.00  & 68.00  & \textbf{74.00 } & 70.00  & \textbf{74.00 } \\
%     miscellaneous & 63.60  & 48.02  & 54.79  & 77.65  & 81.61  & 72.80  & \textbf{81.99 } \\
%     moral disputes & 50.87  & 43.93  & 49.42  & 65.03  & 71.10  & 61.56  & \textbf{71.97 } \\
%     moral scenarios & 23.91  & 28.04  & 31.96  & 29.50  & \textbf{32.51 } & 28.83  & 26.93  \\
%     nutrition & 48.69  & 46.41  & 51.96  & 65.69  & \textbf{75.49 } & 67.65  & \textbf{75.49 } \\
%     philosophy & 59.81  & 45.98  & 50.80  & 67.20  & 69.45  & 66.56  & \textbf{74.28 } \\
%     prehistory & 48.77  & 44.14  & 44.44  & 67.90  & 73.77  & 60.80  & \textbf{75.00 } \\
%     professional accounting & 36.17  & 30.85  & 31.21  & 42.20  & \textbf{48.94 } & 39.36  & 44.68  \\
%     professional law & 36.25  & 32.01  & 36.25  & 41.59  & \textbf{45.11 } & 41.66  & 42.63  \\
%     professional medicine & 52.21  & 40.07  & 41.54  & 58.82  & \textbf{68.38 } & 55.51  & 58.82  \\
%     professional psychology & 43.79  & 36.60  & 41.83  & 59.64  & 67.81  & 58.99  & \textbf{71.08 } \\
%     public relations & 54.55  & 50.91  & 49.09  & 64.55  & \textbf{67.27 } & 64.55  & 66.36  \\
%     security studies & 48.16  & 51.43  & 57.55  & 69.80  & \textbf{72.65 } & 64.49  & 69.80  \\
%     sociology & 62.69  & 47.76  & 67.66  & 79.10  & 83.08  & 69.65  & \textbf{84.08 } \\
%     us foreign policy & 64.00  & 55.00  & 68.00  & 81.00  & \textbf{86.00 } & 75.00  & 82.00  \\
%     virology & 41.57  & 41.57  & 39.76  & 47.59  & \textbf{54.82 } & 45.78  & 53.01  \\
%     world religions & 69.01  & 53.22  & 50.88  & 76.61  & 83.04  & 80.70  & \textbf{83.63 } \\
%     \midrule
%     Average & 46.79  & 40.39  & 47.89  & 59.72  & 64.07  & 57.02  & \textbf{65.71 } \\
%     \bottomrule
%     \end{tabular}%
%   }
%   \caption{xxxx}\label{tab:addlabel}%
% \end{table*}%

==> latex/images/agieval_results.tex <==
\begin{figure}[!tbp]
    \centering
    \includegraphics[width=0.45\textwidth]{image/agieval_results.pdf}
    \caption{Some results in AGIEval benchmark}
    \label{fig:agieval_results}
    \vspace{-0.5cm}
\end{figure}

==> latex/images/data_comparetion.tex <==
\begin{table*}[!htbp]
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c m{5cm}<{\centering} c m{3cm}<{\centering} m{5.5cm}<{\centering} c m{1cm}<{\centering}}
    \toprule
    \textbf{Datasets} & \textbf{Target domain} & \textbf{automatic} & \textbf{methods} & \textbf{source} & \textbf{Data scale} & \textbf{Open Source} \\
    \midrule
    Proof of Pile & Mathematics reasoning  & \XSolidBrush     & \multicolumn{1}{c}{human collection} & arXiv, Textbooks, Lib., Stack Exchange, ProofWiki, MATH & 8.3B  & \Checkmark \\
    OpenWebMath & Mathematics reasoning  & \XSolidBrush     & \multicolumn{1}{c}{human collection} & \multicolumn{1}{c}{Common Crawl} & 14.7B & \Checkmark \\
    MATHPILE & Mathematics reasoning  & \XSolidBrush     & \multicolumn{1}{c}{human collection} & arXiv, Textbooks, Lib., Stack Exchange, ProofWiki, MATH,Web & 9.5B  & \Checkmark \\
    AcademicGPT & Academic & \XSolidBrush     & \multicolumn{1}{c}{human collection} & arXiv, Unpaywall,Top Universities, Pubmed, Common Crawl, Semantic Scholar, Wiki & 370B  & \XSolidBrush \\
    Galactica & Academic & \XSolidBrush     & \multicolumn{1}{c}{human collection} & Papers, Code, Reference Material, Knowledge Bases, Common Crawl, Prompts & 106B  & \XSolidBrush \\
    \knowledgepile~(ours) & Mathematics reasoning \& Knowledge & \Checkmark     & automatic query and retrieve & Public Corpora &  188B  & \Checkmark \\
    \bottomrule
    \end{tabular}
    }
    \caption{Comparation of \knowledgepile with other specific domain knowledge dataset. In this table, most data scales are derived from publicly released research papers, while the data scale for the \knowledgepile~is obtained through tokenized data analysis using the Llama2 tokenizer.}
    \label{tab:data_comparetion}
\end{table*}

==> latex/images/mmlu_results.tex <==
\begin{figure}[t]
    \centering
    % \vspace{-10pt}
    \includegraphics[width=0.47\textwidth]{image/mmlu_results.pdf}
    \caption{The results in MMLU benchmark}
    \label{fig:mmlu_results}
    \vspace{-10pt}
\end{figure}

==> latex/images/query_any.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{image/query_desc.pdf}
    \subcaption{The category distribution of the query for \knowledgepile.}
    \label{fig:pie_query_domain}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{image/qoc_collection.pdf}
    \subcaption{}
    \label{fig:}
    \end{subfigure}
\end{figure}



==> latex/images/query_of_cc_timestamp.tex <==
\begin{figure}[!tbp]
    \centering
    \includegraphics[width=0.4\textwidth]{image/query_of_cc_timestamp_prop.pdf}
    \caption{Timestamp Statistics of \knowledgepile}
    \label{fig:queryofcc_timestamp}
    \vspace{-10pt}
\end{figure}

==> latex/images/web_domain_timestamp.tex <==
\begin{figure}
    \begin{subfigure}[b]{0.5\textwidth}
        \begin{tabular}{lc}
        \toprule
        \textbf{Web Domain} & \textbf{Count} \\
        \midrule
        en.wikipedia.org & 398833 \\
        www.semanticscholar.org & 141268 \\
        slideplayer.com & 108177 \\
        www.ncbi.nlm.nih.gov & 97009 \\
        link.springer.com & 85357 \\
        www.ipl.org & 84084 \\
        pubmed.ncbi.nlm.nih.gov & 68934 \\
        www.reference.com & 61658 \\
        www.bartleby.com & 60097 \\
        quizlet.com & 56752 \\
        \bottomrule
        \end{tabular}
      \caption{Top 10 web domain of \knowledgepile}\label{tab:webdomain}
    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \includegraphics[width=.8\textwidth]{image/query_of_cc_timestamp_prop.pdf}
        \caption{Timestamp Statistics of \knowledgepile}
        \label{fig:queryofcc_timestamp}
    \end{subfigure}
\end{figure}
